CoMA: Compositional Human Motion Generation with Multi-modal Agents

3D human motion generation has seen substantial advancement in recent years. While state-of-the-art approaches have improved performance significantly, they still struggle with complex and detailed motions unseen in training data, largely due to the scarcity of motion datasets and the prohibitive cost of generating new training examples. To address these challenges, we introduce CoMA, an agent-based solution for complex human motion generation, editing, and comprehension. CoMA leverages multiple collaborative agents powered by large language and vision models, alongside a mask transformer-based motion generator featuring body part-specific encoders and codebooks for fine-grained control. Our framework enables generation of both short and long motion sequences with detailed instructions, text-guided motion editing, and self-correction for improved quality. Evaluations on the HumanML3D dataset demonstrate competitive performance against state-of-the-art methods. Additionally, we create a set of context-rich, compositional, and long text prompts, where user studies show our method significantly outperforms existing approaches.

==> figs/coma_workflow_example.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{imgs/coma_workflow_example.png}
    \caption{This figure spans both columns in a two-column document.}
    \label{fig:coma_workflow_example}
\end{figure*}

==> preamble.tex <==
%
% --- inline annotations
%




==> prompts/traj_gen.tex <==
\begin{tcolorbox}[
    breakable,
    colback=white,
    colframe=black,
    boxrule=0.5pt,
    left=5pt,
    right=5pt,
    top=5pt,
    bottom=5pt
]
\begin{minted}[
    fontsize=\scriptsize,
    breaklines=true,
    tabsize=4,
    breakanywhere=true
]{text}
**Task:** Draw a continuous trajectory to represent a specified curve/line/shape(trajectory) of a person, according to the given [Description].

**YOUR OUTPUT SHOULD CONTAIN:**

1. **Closed or Open Trajectory Decision:** Decide if the trajectory is closed or open based on the description. For example, if it's a geometric figure or involves "walking around," it's likely closed. If it's a path like the letter 'S', 'L', etc., it's open. So, avoid using a closed trajectory for an open path like S, a common error is to make it like shape 8.

2. **Extract the Trajectory Using Fixed Format Breakdown: (ONLY DO WHEN Trajectoy is complex or vague. If it's simple, you can skip this step)** Break down the action description into simple, precise steps. Use a fixed format to describe the movement (e.g., "Walk forward for 5 meters, then turn 90 degrees right"). This helps in extracting the trajectory.

2.1 Avoid overcomplicating the movement.Keep it accurate and straightforward.

3. **Trajectory Analysis:** Analyze the described trajectory before writing the code. Consider overlapping parts where necessary (it's not normal curve, it's trajectory. A man's trajectory can overlap). The parameter `t` in `shape_curve(t)` may represent time in some cases.

Note: Your understanding of clock directions might be different from mine, so here's a quick reference:
12 o'clock: Straight ahead
3 o'clock: Directly to your right
6 o'clock: Directly behind you
9 o'clock: Directly to your left
1-2 o'clock: Slightly to the right front
10-11 o'clock: Slightly to the left front
4-5 o'clock: Slightly to the right back
7-8 o'clock: Slightly to the left back

Note: Whether it's to the right, left, or any clock direction, it's always referenced from the perspective of the person walking this trajectory, not from the image's perspective.

**Note:** Clock directions are always referenced from the perspective of the person performing the trajectory.
Ensure that both x and y coordinates change uniformly over time (`t`). This means the trajectory should reflect a consistent speed of movement.
To ensure no "instant jumps" in the generated trajectory, specify that the trajectory function must have smooth transitions between segments. Emphasize continuity, meaning each segment's start must align with the previous segment's end, avoiding abrupt shifts. Additionally, ensure uniform speed across the entire range of `t`, with x and y coordinates changing evenly over time.

Emphasize once again: To ensure a smooth transition, you need to adjust the formulas for each segment so that they start from the endpoint coordinates of the previous segment, rather than independently redefining ( x ) and ( y ). If there are multiple segments, the starting and ending coordinates for each segment should be clearly marked in the comments as **start_x, start_y, end_x, end_y**.
Emphasize once again: To ensure a smooth transition, you need to adjust the formulas for each segment so that they start from the endpoint coordinates of the previous segment, rather than independently redefining \( x \) and \( y \). If there are multiple segments, the starting and ending coordinates for each segment should be clearly marked in the comments as **start_x, start_y, end_x, end_y**.

4. **Mathematical Functions:** Present the final code strictly in the form provided below, ensuring it is correct and can run without errors and READY TO USE.

**Code Format:**
```python
def shape_curve(t):xz
    ...

    return x, y

# Specify the range of t (it is important)
t_range = (start_value, end_value)
```

---

Now the input is:

- [ ] "I want to draw a Description = 'placeholder1'. Give me `def shape_curve(t)`."

\end{minted}
\end{tcolorbox}
